RESTOR: Knowledge Recovery in Machine Unlearning

Large language models trained on web-scale corpora can memorize undesirable data containing misinformation, copyrighted material, or private or sensitive information. Recently, several machine unlearning algorithms have been proposed to eliminate the effect of such datapoints from trained models -- that is, to approximate a model that had never been trained on these datapoints in the first place. However, evaluating the effectiveness of unlearning algorithms remains an open challenge. Previous work has relied on heuristics -- such as verifying that the model can no longer reproduce the specific information targeted for removal while maintaining accuracy on unrelated test data. These approaches inadequately capture the complete effect of reversing the influence of datapoints on a trained model. In this work, we propose the RESTOR framework for machine unlearning evaluation, which assesses the ability of unlearning algorithms for targeted data erasure, by evaluating the ability of models to forget the knowledge introduced in these datapoints, while simultaneously recovering the model's knowledge state had it never encountered these datapoints. RESTOR helps uncover several novel insights about popular unlearning algorithms, and the mechanisms through which they operate -- for instance, identifying that some algorithms merely emphasize forgetting but not recovering knowledge, and that localizing unlearning targets can enhance unlearning performance.

==> sections/figures/logits.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.46\textwidth]{sections/figures/logits_file.pdf}
    \vspace{-8pt}
    \caption{Probability distributions of clean, corrupted, and unlearned models across output categories: clean, corrupted, and random. NPO restores clean probabilities by lowering corrupted ones, while GA shifts corrupted probabilities toward random outputs.
    }
    \label{fig:logits}
    \vspace{-10pt}
\end{figure}

==> sections/tables/corruption.tex <==
\begin{table}
\centering
% \ar{Can we move caption below table. In *CL both table and figure captions go below.}}
% \begin{tabular}{l|c}
% Model       & Accuracy \\ \hline \hline
% $\clean$                          & 65.84          \\ \hline
% $\corrupted$ $(k=0)$              & 61.46          \\ \hline
% $\corrupted$ $(k=1)$              & 50.71          \\ %\hline
% $\corrupted$ $(k=2)$              & 49.35          \\ %\hline
% $\corrupted$ $(k=3)$              & 50.36          \\ %\hline
% $\corrupted$ $(k=4)$              & 45.72          \\ %\hline
% $\corrupted$ $(k=5)$              & 44.45          \\ %\hline
% \end{tabular}
% \begin{tabular}{c|c}
% Model       & Accuracy \\ \hline \hline
% $\clean$                          & 65.84          \\ \hline
% $\corrupted$ $(k=0)$              & 61.46 \footnotesize{\textcolor{red}{(-4.38)}}          \\ \hline
% $\corrupted$ $(k=1)$              & 50.71 \footnotesize{\textcolor{red}{(-15.13)}}         \\ %\hline
% $\corrupted$ $(k=2)$              & 49.35 \footnotesize{\textcolor{red}{(-16.49)}}         \\ %\hline
% $\corrupted$ $(k=3)$              & 50.36 \footnotesize{\textcolor{red}{(-15.48)}}         \\ %\hline
% $\corrupted$ $(k=4)$              & 45.72 \footnotesize{\textcolor{red}{(-20.12)}}         \\ %\hline
% $\corrupted$ $(k=5)$              & 44.45 \footnotesize{\textcolor{red}{(-21.39)}}         \\ %\hline
% \end{tabular}
\begin{tabular}{l|c|c}
                             \multicolumn{2}{c|}{Model}       & Accuracy \\ \hline \hline
                             \multicolumn{2}{c|}{$\clean$}                          & 65.84          \\ \hline
\multirow{6}{*}{$\corrupted$} & $k=0$              & 61.46 \footnotesize{\textcolor{red}{(-4.38)}}          \\ %\cline{2-3}
                             & $k=1$              & 50.71 \footnotesize{\textcolor{red}{(-15.13)}}         \\ %\hline
                             & $k=2$              & 49.35 \footnotesize{\textcolor{red}{(-16.49)}}         \\ %\hline
                             & $k=3$              & 50.36 \footnotesize{\textcolor{red}{(-15.48)}}         \\ %\hline
                             & $k=4$              & 45.72 \footnotesize{\textcolor{red}{(-20.12)}}         \\ %\hline
                             & $k=5$              & 44.45 \footnotesize{\textcolor{red}{(-21.39)}}         \\ %\hline
\end{tabular}
\caption{Corruption datasets can effectively degrade model's performance on factual questions.
$k$ controls the amount of unrelated context in corruption datasets, more unrelated context leads to more severe corruption.
% \fb{mention what's K again}
}
\label{tab:corruption}
\end{table}

==> sections/tables/unaffected.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{l|cc}
        \toprule
        Method & {\footnotesize Degradation (\%)} & {\footnotesize Unaffected (\%)} \\
        \midrule
        NPO & 3.65 & 96.35\\
        KL  & 26.26 & 73.74\\
        GA  & 32.12 & 67.88\\
        \bottomrule
    \end{tabular}
    \caption{Performance of unlearned models on questions where both clean and corrupted models predict correctly. NPO better preserves remaining knowledge in corrupted model, while GA and KL risk degrading that.
    % ($k=4$ for the corruption dataset).
    }
    \label{tab:unaffected}
    \vspace{-5pt}
\end{table}

